Multimodality in the Hypergraph Lambek Calculus

The multimodal Lambek calculus is an extension of the Lambek calculus that includes several product operations (some of them being commutative or/and associative), unary modalities, and corresponding residual implications. In this work, we relate this calculus to the hypergraph Lambek calculus HL. The latter is a general pure logic of residuation defined in a sequent form; antecedents of its sequents are hypergraphs, and the rules of HL involve hypergraph transformation. Our main result is the embedding of the multimodal Lambek calculus (with at most one associative product) in HL. It justifies that HL is a very general Lambek-style logic and also provides a novel syntactic interface for the multimodal Lambek calculus: antecedents of sequents of the multimodal Lambek calculus are represented as tree-like hypergraphs in HL, and they are derived from each other by means of hyperedge replacement. The advantage of this embedding is that commutativity and associativity are incorporated in the sequent structure rather than added as separate rules. Besides, modalities of the multimodal Lambek calculus are represented in HL using the product and the division of HL, which explicitizes their residual nature.

==> eptcsdata.tex <==
\providecommand{\firstpage}{46}
\providecommand{\publicationstatus}{M. Moortgat and M. Sadrzadeh (Eds.): Modalities in substructural logics.\\
Applications at the interfaces of logic, language and computation (AMSLO 2023).\\
EPTCS 381, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.381.6}{10.4204/EPTCS.381.6}}

